What Matters in Learning from Offline Human Demonstrations for Robot Manipulation

Imitating human demonstrations is a promising approach to endow robots with various manipulation capabilities. While recent advances have been made in imitation learning and batch (offline) reinforcement learning, a lack of open-source human datasets and reproducible learning methods make assessing the state of the field difficult. In this paper, we conduct an extensive study of six offline learning algorithms for robot manipulation on five simulated and three real-world multi-stage manipulation tasks of varying complexity, and with datasets of varying quality. Our study analyzes the most critical challenges when learning from offline human data for manipulation. Based on the study, we derive a series of lessons including the sensitivity to different algorithmic design choices, the dependence on the quality of the demonstrations, and the variability based on the stopping criteria due to the different objectives in training and evaluation. We also highlight opportunities for learning from human datasets, such as the ability to learn proficient policies on challenging, multi-stage tasks beyond the scope of current reinforcement learning methods, and the ability to easily scale to natural, real-world manipulation scenarios where only raw sensory signals are available. We have open-sourced our datasets and all algorithm implementations to facilitate future research and fair comparisons in learning from human demonstration data. Codebase, datasets, trained models, and more available at https://arise-initiative.github.io/robomimic-web/

==> 1-intro.tex <==
\section{Introduction}
\label{sec:intro}

% Much of the recent progress in AI and Machine Learning is rooted in the ability to pose tasks as supervised learning problems~\cite{bishop2006pattern}.
% By extracting information from human-labeled data, computer vision and natural language processing algorithms have been able to solve decades-old problems~\cite{}.
% In imitation learning (IL), the same paradigm is applied to train robots to reproduce human performance in physical tasks. 
% However, despite significant advances~\cite{}, the results of IL in robot manipulation tasks have not been yet as disruptive as we observe other disciplines.
% What makes imitation learning for robot manipulation from human demonstrations so hard?

%Here, the main issues. Map to the issues you evaluate in experiments


\yuke{Selling human supervision is a non-starter as it sounds lame for ML audience. I'd rephrase this paragraph to say that albeit significant incentives have dedicated to devising algorithms that learn from less supervision, the state-of-the-art performances are typically obtained from high-quality human supervision.} 
Human supervision has been at the heart of incredible recent advances in several domains such as Computer Vision~\cite{deng2009imagenet} and Natural Language Processing~\cite{rajpurkar2018squad2}. By intelligently leveraging large datasets annotated by humans, autonomous machines have been able to reach near-human performance on several tasks such as image recognition and question-answering. Unfortunately, achieving similar success in robotics by using human supervision remains an open problem.

% P2: there have been attempts to use human supervision for robotics, and in fact in many different ways, like demos, feedback, corrections, etc. (end-to-end data-driven methods super promising, give examples of IL like we have currently) MDP-like setting has been super promising. But the kinds of tasks that robots can do are still limited in many ways, and are nowhere near the complexity of tasks that human-level intelligence can solve with ease.
There have been several different attempts to leverage human supervision for robotics. Unlike other domains, human supervision in robotics can come in many different forms\yuke{Other domains, e.g., CV and NLP, might also have drastically different forms of supervision. Use a better sentence to describe how the form of supervision in robotics is different (hint: it's a time-evolving dynamical system)} -- prior work has tried using human supervision in the form of human demonstrations provided both by teleoperating the robot~\cite{zhang2017deep, mandlekar2020learning} and via kinesthetic teaching~\cite{hersch2008dynamical, kormushev2011imitation, akgun2012trajectories}, corrections to actions taken by the robot~\cite{ross2011reduction, bajcsy2017learning, bajcsy2018learning, mandlekar2020human}, and positive and negative feedback for robot actions~\cite{zhang2019leveraging, loftin2016learning, macglashan2017interactive, cabi2019scaling, christiano2017deep, singh2019end}. End-to-end data-driven approaches have emerged as a promising way to endow robots with various manipulation capabilities from human demonstrations. Recent methods have enabled robots to perform tasks such as insertion~\cite{ddpgfd}, picking, placing, and pushing items~\cite{zhang2017deep}, hanging a cap on a rack~\cite{florence2019self}, and putting items into an oven for baking~\cite{mandlekar2020learning}. However, the abilities of autonomous robots are still limited in critical ways compared to the wide range of tasks that humans can solve effortlessly using physical and cognitive intelligence.

% TODO: do we need the first part of this paragraph anymore?
% P3: some of the difficulties are that human supervision can come in many forms, and can be much more unstructured than other domains (both how to collect, and how to use / learn from it. To try and replicate successes from other domains, we need to study this setting more extensively!
Learning from human demonstration data in such settings could help bridge this gap between robot and human intelligence.\yuke{More motivation on \textbf{offline} and \textbf{human-provided} datasets - you used the word \textbf{human-provided} several times but I feel that the message did not come across because there is no contrast (what is not human-provided, i.e., agent-generated) and insufficient explanation on the value of human data} Consequently, studying how robots can learn effectively from human-provided datasets is an important problem. Unfortunately, a lack of open-source human datasets and reproducible learning methods make studying this setting difficult.\yuke{explain why it's hard - like no scalable methods to collect such data from hihg-DoF arms, learning methods are sensitive to tunable knobs, etc.} While it is indeed possible to collect large-scale human demonstration datasets~\cite{sharma2018multiple, mandlekar2018roboturk, mandlekar2019scaling}, reproducible studies on human demonstration datasets are missing.

% P4: But studying this setting is difficult for researchers today! Let's take an initial step towards addressing this large problem, by collecting several datasets via teleoperation and trying to learn from them, in RL-like setting. 
In this paper, we address this need by presenting a study of data-driven offline policy learning methods on several human-provided robot manipulation datasets. We collect task demonstrations from human teleoperators across a broad range of simulated and real world manipulation tasks and investigate different factors that play a substantial role in learning from such data. 

% P5: Here are some factors that we explore in our study, using agent-generated data as a baseline. By studying these factors, we learned about several challenges, opportunities, and lessons in learning from offline human demonstrations that will be critical for the research community.
Some factors that we study include the importance of model architecture, performance differences between single and multi-human datasets, how batch (offline) reinforcement learning performs on suboptimal human datasets, the role of observation space and hyperparameter selection in training performant policies from human data, and the ability of algorithms to scale to challenging, real-world settings. We also compare to agent-generated datasets (which are increasingly prevalent in recent offline policy learning benchmarks~\cite{fu2020d4rl, gulcehre2020rl} \yuke{consider moving this to earlier paragraphs for motivation}) where appropriate, to underscore differences in learning from human datasets. From our results, we point out several challenges, opportunities, and lessons in learning from offline human demonstrations that will hopefully guide future research in leveraging human supervision for robot manipulation effectively.

% P6: Summarize a handful of best insights, and then list contributions.
We find that design choices such as the agent architecture, choice of observation space for a task, and hyperparameters for each learning algorithm play a large role in learning proficiency, and state-of-the-art algorithms, while very proficient on agent-generated datasets, are unable to properly leverage suboptimal human data. To enable learning from larger human datasets, provided by several different possibly suboptimal human supervisors, it is important for future work to focus on addressing such challenges. We also find that human datasets can be a viable approach to solve multi-stage challenging manipulation tasks beyond the scope of current data-driven methods, and that our insights from simulation can be applied directly to solve real-world tasks. Consequently, learning from human datasets like the ones provided in this study holds promise for extending the range of capabilities for autonomous robots.

\noindent \textbf{Summary of Contributions:}
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    leftmargin=*,
    itemindent=12pt]
\item We present an empirical study of data-driven offline policy learning algorithms across several human-provided robot manipulation datasets with five challenging simulated tasks and three real world tasks.
\item We summarize our insights from our study into challenges, opportunities, and lessons to guide future work in learning from human-provided datasets.
\end{enumerate}



% We can help address this by collecting several datasets (enabled by RoboTurk!) and conducting a study to investigate what matters. By doing so, we hope to reveal some challenges and opportunities in learning from human data, to guide future research.

% Such studies would enable researchers to develop better algorithms to learn from human data without facing the burden of collecting their own datasets. 
% Furthermore, having datasets that disentangle the challenge of learning from different dataset sources, different observation spaces, and different task complexities would help provide more confidence in results.

% Open-source everything to make sure people can reproduce and build on top of our stuff!

% Summarize surprising findings, and then properly state contributions.

==> 6-related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Human Supervision for Robotics:} Prior work has tried using human supervision in the form of human demonstrations provided both by teleoperating the robot~\cite{zhang2017deep, mandlekar2020learning} and via kinesthetic teaching~\cite{hersch2008dynamical, kormushev2011imitation, akgun2012trajectories}, corrections to actions taken by the robot~\cite{ross2011reduction, bajcsy2017learning, bajcsy2018learning, mandlekar2020human}, and positive and negative feedback for robot actions~\cite{zhang2019leveraging, loftin2016learning, macglashan2017interactive, cabi2019scaling, christiano2017deep, singh2019end}.

% \textbf{Offline Learning from Demonstrations}: Imitation Learning (IL) is a popular paradigm for training policies from a set of demonstrations. Offline Imitation Learning typically consists of variants of Behavioral Cloning (BC)~\cite{pomerleau1989alvinn}, where a policy is trained to output the same actions as the ones taken by the demonstrator in each state. Offline IL has been used extensively in robotic manipulation~\cite{Ijspeert2002MovementIW, Finn2017OneShotVI, Billard2008RobotPB, Calinon2010LearningAR, zhang2017deep, mandlekar2020learning, zeng2020transporter, wang2021generalization, tung2020learning}. Typically, IL assumes that the demonstration data is optimal. By contrast, Batch (Offline) Reinforcement Learning~\cite{lange2012batch, levine2020offline} is a method to learn from demonstrations that can consist of both good and bad quality data, by leveraging reward annotations in the datasets. Prior algorithms~\cite{fujimoto2019off, kumar2020conservative, wu2019behavior, wang2020critic, siegel2020keep, kidambi2020morel, yu2020mopo, ghasemipour2020emaq, yu2021combo} are mostly evaluated on datasets generated by several RL-trained policies of varying quality. In this study, we evaluate both offline IL and offline RL algorithms on datasets collected from one or more humans, which can both break the assumption of optimality in IL, and present interesting challenges for offline RL methods compared to commonly used RL-generated datasets. 

\textbf{Empirical Studies in Reinforcement and Imitation Learning}: % There are several prior studies that explore how design choices can affect reinforcement learning in different domains. 
Prior work has benchmarked Reinforcement Learning (RL) algorithms in continuous control domains~\cite{duan2016benchmarking}, run extensive evaluations of model-based RL algorithms~\cite{wang2019benchmarking} and on-policy RL methods~\cite{andrychowicz2020matters}, and shown how Deep RL algorithms can be extremely sensitive to hyperparameter choices and can make reproducing results challenging~\cite{henderson2018deep}. There are fewer empirical studies in imitation learning. The MAGICAL benchmark~\cite{toyer2020magical} consists of 2D environments that test the ability of IL algorithms to generalize. Both RLBench~\cite{james2020rlbench} and Ravens~\cite{zeng2020transporter} provide several simulated robot manipulation tasks and expert demonstrations for imitation learning, but demonstrators are pre-programmed and rely on ground-truth simulator state. 
% By contrast, our datasets are collected by humans that directly teleoperate robot arms in both simulated and real-world settings from pure visual observations. 
Simitate~\cite{memmesheimer2019simitate} is an imitation learning benchmark suite consisting of real-world motion trajectories collected by humans, and carefully translated into simulation using extensive sensor instrumentation in the real world. 
By contrast, our datasets are collected via remote teleoperation from humans in both simulated and real-world settings, allowing fast and easy demonstration collection for a wide range of tasks without assuming privileged instrumentation. 
% Recently, Hussenot et al.~\cite{hussenot2021hyperparameter} presented an empirical study on the importance of hyperparameter selection in imitation learning -- it consists of an extensive evaluation of both offline and online imitation learning algorithms using modest-sized datasets (\textasciitilde10s of trajectories). This work is complementary to ours -- we also confirm the importance of hyperparameter selection when learning offline from human-provided datasets (\textasciitilde100s of trajectories).
Recently, Hussenot et al.~\cite{hussenot2021hyperparameter} presented an empirical study on the importance of hyperparameter selection in imitation learning -- this work is complementary to ours.
% In this paper, we evaluate offline imitation and reinforcement learning algorithms on human-provided datasets in physically complex robot manipulation tasks.

\textbf{Robot Manipulation Benchmarks}: Several benchmark robot manipulation tasks have been proposed before~\cite{fan2018surreal, lin2020softgym, yu2020meta, robosuite2020, james2020rlbench, ahmed2020causalworld}. Benchmark datasets~\cite{fu2020d4rl, gulcehre2020rl} have also been proposed recently for batch (offline) reinforcement learning. While these datasets span a variety of domains (locomotion, control, autonomous driving, video games, robot manipulation), most of the datasets are generated by autonomous agents trained with online reinforcement learning. Unfortunately, this means that most of these datasets are limited to tasks that RL methods can solve from scratch. By contrast, we focus on datasets collected by one or more humans, allowing us to increase the complexity of the tasks we consider. Furthermore, our study explores how learning from human data can be substantially different than agent datasets.



==> 7-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Going forward, we hope that the datasets, tasks, code, and subsequent insights of our study will serve researchers and practitioners alike.

==> A-errata.tex <==
\section{Errata}
\label{app:errata}

\begin{enumerate}
    \item Fig~\ref{fig:hyper-image} x-axis label should say "shallow Conv" instead of "larger MLP".
\end{enumerate}

==> fig-tasks-real.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{figures/task_6.pdf}
\caption{Lift} 
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{figures/task_7.pdf}
\caption{Pick Place Can} 
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{figures/task_8.pdf}
\caption{Tool Hanging} 
\end{subfigure}
\begin{subfigure}{0.39\textwidth}
% \begin{table}
\small
\caption{\textbf{Real Robot Results}}
\label{table:real_robot}
\centering
\begin{tabular}{cc}
\toprule
\textbf{Task} & 
\begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} \\
\midrule

Lift & 96.7 \\ % 29 out of 30
Pick Place Can & 73.3 \\ % 22 out of 30
Tool Hanging & - \\

\bottomrule
\end{tabular}
% \end{table}
\end{subfigure}
\caption{\textbf{Real World Tasks and Results} We present 3 challenging manipulation tasks.}
\label{fig:real_benchmark_tasks}
\vspace{-15pt}
\end{figure}

==> tab-hypers_old.tex <==
\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Proficient-Human (PH) Hyperparameters - Low Dim (LD) Observations}}
  \label{tab:hypers-se-ld}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    \multirow{9}{*}{GTI}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \midrule
    
    \multirow{5}{*}{IRIS}
    & Base Template & GTI-PH-LD \\
    & Planner LR & $1e-3$ \\
    & Actor LR & $1e-3$ \\
    & Value LR & $1e-3$ \\
    & Value KL & $0.5$ \\
    \midrule
    
    \multirow{5}{*}{CQL}
    & Q network LR & $1e-3$ \\
    & Policy LR & $3e-4$ \\
    & Deterministic Backup & True \\
    & Batch Size & $1024$ \\
    & Lagrange & True \\
    & Lagrange Threshold $\tau$ & $5.0$ \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}

\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Proficient-Human (PH) Hyperparameters - Image (IM) Observations}}
  \label{tab:hypers-se-im}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}

\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Multi-Human (MH) Hyperparameters - Low Dim (LD) Observations}}
  \label{tab:hypers-mh-ld}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    \multirow{1}{*}{GTI}
    & Base Template & GTI-PH-LD \\
    \midrule
    
    \multirow{5}{*}{IRIS}
    & Base Template & GTI-MH-LD \\
    & Planner LR & $1e-3$ \\
    & Actor LR & $1e-3$ \\
    & Value LR & $1e-4$ \\
    & Value KL & $0.05$ \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}

\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Multi-Human (MH) Hyperparameters - Image (IM) Observations}}
  \label{tab:hypers-mh-im}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}


\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Machine-Generated (MG) Hyperparameters - Low Dim (LD) Observations}}
  \label{tab:hypers-rb-ld}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    \multirow{3}{*}{GTI}
    & Base Template & GTI-PH-LD \\
    & Actor RNN Hidden Dim & $100$ \\
    & Actor MLP Dims & $[1024, 1024]$ \\
    \midrule
    
    \multirow{5}{*}{IRIS}
    & Base Template & GTI-MG-LD \\
    & Planner LR & $1e-3$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    & Value LR & $1e-3$ \\
    & Value KL & $0.5$ \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}

\begin{table*}
  \fontsize{8}{10}\selectfont
  \caption{\textbf{Machine-Generated (MG) Hyperparameters - Image (IM) Observations}}
  \label{tab:hypers-rb-im}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Algorithm & Hyperparameter & Value \\
    \midrule
    
    % Fill in the number below corresponding to number of hypers you're specifying for your algo
    \multirow{10}{*}{YOUR ALGO}
    & Base Template & Default \\
    & Planner LR & $1e-3$ \\
    & Planner VAE KL & $5e-4$ \\
    & Planner VAE GMM Prior & True \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE GMM Latent Dim & $16$ \\
    & Planner VAE MLP Dims & $[1024, 1024]$ \\
    & Actor LR & $1e-3$ \\
    & Actor RNN Hidden Dim & $400$ \\
    & Actor MLP Dims & $[]$ \\
    \bottomrule
  \end{tabular}
\vspace{-15pt}
\end{table*}

==> tables/table-core-image.tex <==
% collect tables to display side-by-side
\begin{table}[t!]
  \small
  \centering
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-core-se-image}
  }
  \hfill
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-core-mh-image}
  }
\end{table}

==> tables/table-core-low-dim.tex <==
% collect tables to display side-by-side
\begin{table}[t!]
  \small
  \centering
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-core-se-low-dim}
  }
  \hfill
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-core-mh-low-dim}
  }
\end{table}

==> tables/table-core-mh-image.tex <==
% \begin{table}
%   \small
%   \caption{\textbf{Proficient Human Results (image)}}
%   \label{table:ph_low_dim}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     \textbf{Task} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC}\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BCQ}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{CQL}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{HBC}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{IRIS}\end{tabular} \\ 
%     \midrule
    
%     Lift & - & - & - & - & - & - \\
%     Can & - & - & - & - & - & - \\
%     Square & - & - & - & - & - & - \\
%     Transport & - & - & - & - & - & - \\
    
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}
\small
\caption{\textbf{Multi Human Results (image)}}
\label{table:mh_image}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Algo} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Lift}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Can}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Square}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Transport}\end{tabular} \\ 
\midrule

BC & - & - & - & - \\
BC-RNN & - & - & - & - \\
BCQ & - & - & - & - \\
CQL & - & - & - & - \\

\bottomrule
\end{tabular}
% \end{table}

==> tables/table-core-mh-low-dim.tex <==
% \begin{table}
%   \small
%   \caption{\textbf{Proficient Human Results (low-dim)}}
%   \label{table:ph_low_dim}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     \textbf{Task} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC}\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BCQ}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{CQL}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{HBC}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{IRIS}\end{tabular} \\ 
%     \midrule
    
%     Lift & - & - & - & - & - & - \\
%     Can & - & - & - & - & - & - \\
%     Square & - & - & - & - & - & - \\
%     Transport & - & - & - & - & - & - \\
    
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}
\small
\caption{\textbf{Multi Human Results (low-dim)}}
\label{table:mh_low_dim}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Algo} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Lift}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Can}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Square}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Transport}\end{tabular} \\ 
\midrule

% BC & $100.0\pm0.0$ & $86.0\pm4.3$ & $52.7\pm6.6$ & $11.3\pm2.5$ \\
% BC-RNN & $100.0\pm0.0$ & $100.0\pm0.0$ & $78.0\pm4.3$ & $65.3\pm7.4$ \\
% BCQ & - & - & - & - \\
% CQL & - & - & - & - \\
% GTI & - & - & - & - \\
% IRIS & - & - & - & - \\

BC & $100.0$ & $86.0$ & $52.7$ & $11.3$ \\
BC-RNN & $100.0$ & $100.0$ & $78.0$ & $65.3$ \\
BCQ & - & - & - & - \\
CQL & - & - & - & - \\
GTI & - & - & - & - \\
IRIS & - & - & - & - \\

\bottomrule
\end{tabular}
% \end{table}

==> tables/table-core-rb-low-dim.tex <==
\begin{table}[t!]
\small
\caption{\textbf{Autonomous Agent Results (low-dim)}}
\label{table:rb_low_dim}
\centering
\begin{tabular}{ccccccc}
\toprule
\textbf{Dataset} & 
\begin{tabular}[c]{@{}c@{}}\textbf{BC}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{BCQ}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{CQL}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{GTI}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{IRIS}\end{tabular} \\ 
\midrule

Lift & $65.3\pm2.5$ & $70.7\pm3.4$ & - & - & - & - \\
Can & $82.0\pm0.0$ & $86.0\pm1.6$ & - & - & - & - \\

% Lift & $65.3$ & $70.7$ & - & - & - & - \\
% Can & $82.0$ & $86.0$ & - & - & - & - \\

% Lift (AA) & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ \\
% Can (AA) & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ \\
% Square (AA) & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ \\
% Transport (AA) & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ & $100.0\pm 10.0$ \\

\bottomrule
\end{tabular}
\end{table}

==> tables/table-core-se-image.tex <==
% \begin{table}
%   \small
%   \caption{\textbf{Proficient Human Results (image)}}
%   \label{table:ph_low_dim}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     \textbf{Task} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC}\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BCQ}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{CQL}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{HBC}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{IRIS}\end{tabular} \\ 
%     \midrule
    
%     Lift & - & - & - & - & - & - \\
%     Can & - & - & - & - & - & - \\
%     Square & - & - & - & - & - & - \\
%     Transport & - & - & - & - & - & - \\
    
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}
\small
\caption{\textbf{Proficient Human Results (image)}}
\label{table:ph_image}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Algo} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Lift}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Can}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Square}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Transport}\end{tabular} \\ 
\midrule

BC & - & - & - & - \\
BC-RNN & - & - & - & - \\
BCQ & - & - & - & - \\
CQL & - & - & - & - \\

\bottomrule
\end{tabular}
% \end{table}

==> tables/table-core-se-low-dim.tex <==
% \begin{table}
%   \small
%   \caption{\textbf{Proficient Human Results (low-dim)}}
%   \label{table:ph_low_dim}
%   \centering
%   \begin{tabular}{ccccccc}
%     \toprule
%     \textbf{Task} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC}\end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{BCQ}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{CQL}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{HBC}\end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{IRIS}\end{tabular} \\ 
%     \midrule
    
%     Lift & - & - & - & - & - & - \\
%     Can & - & - & - & - & - & - \\
%     Square & - & - & - & - & - & - \\
%     Transport & - & - & - & - & - & - \\
    
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}
\small
\caption{\textbf{Proficient Human Results (low-dim)}}
\label{table:ph_low_dim}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{Algo} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Lift}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Can}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Square}\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Transport}\end{tabular} \\ 
\midrule

% BC & $100.0\pm0.0$ & $95.3\pm0.9$ & $78.7\pm1.9$ & $17.3\pm2.5$ \\
% BC-RNN & $100.0\pm0.0$ & $100.0\pm0.0$ & $84.0\pm0.0$ & $71.3\pm6.6$ \\
% BCQ & - & - & - & - \\
% CQL & - & - & - & - \\
% GTI & - & - & - & - \\
% IRIS & - & - & - & - \\

BC & $100.0$ & $95.3$ & $78.7$ & $17.3$ \\
BC-RNN & $100.0$ & $100.0$ & $84.0$ & $71.3$ \\
BCQ & - & - & - & - \\
CQL & - & - & - & - \\
GTI & - & - & - & - \\
IRIS & - & - & - & - \\

\bottomrule
\end{tabular}
% \end{table}

==> tables/table-ds-size-low-dim.tex <==
% collect tables to display side-by-side
\begin{table}[t!]
  \small
  \centering
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-ds-size-low-dim-se}
  }
  \hfill
  \parbox[t][][t]{.49\linewidth}{
  \input{tables/table-ds-size-low-dim-mh}
  }
\end{table}


==> tables/table-real.tex <==
% \begin{table}
\begin{wraptable}{r}{4.0cm}
\small
\centering
\begin{tabular}{cc}
\toprule
\textbf{Task} & 
\begin{tabular}[c]{@{}c@{}}\textbf{BC-RNN}\end{tabular} \\
\midrule

Lift & 96.7 \\ % 29 out of 30
Can & 73.3 \\ % 22 out of 30
Can (- Rand) & 26.7 \\ % 8 out of 30
Can (- Wrist) & 43.3 \\ % 13 out of 30
Tool Hang & - \\

\bottomrule
\end{tabular}
\caption{\textbf{Real Robot Results} BC-RNN learns proficient real-world policies. Pixel-shift randomization and wrist observations are crucial.}
\label{table:real}
\end{wraptable}
% \end{table}

==> tables/table-th.tex <==
% \begin{table}
\begin{wraptable}{r}{5.5cm}
\small
\caption{\textbf{Tool Hang Results}}
\label{table:tool}
\centering
\begin{tabular}{ccc}
\toprule
\textbf{Algo} & 
\begin{tabular}[c]{@{}c@{}}\textbf{Low-dim}\end{tabular} &
\begin{tabular}[c]{@{}c@{}}\textbf{Image}\end{tabular} \\
\midrule

BC & - & - \\
BC-RNN & - & - \\
BCQ & - & - \\
CQL & - & - \\
HBC & - & - \\
IRIS & - & - \\

\bottomrule
\end{tabular}
\end{wraptable}
% \end{table}
